Compressive Multiplexing of Correlated Signals

We present a general architecture for the acquisition of ensembles of correlated signals. The signals are multiplexed onto a single line by mixing each one against a different code and then adding them together, and the resulting signal is sampled at a high rate. We show that if the $M$ signals, each bandlimited to $W/2$ Hz, can be approximated by a superposition of $R < M$ underlying signals, then the ensemble can be recovered by sampling at a rate within a logarithmic factor of $RW$ (as compared to the Nyquist rate of $MW$). This sampling theorem shows that the correlation structure of the signal ensemble can be exploited in the acquisition process even though it is unknown a priori. The reconstruction of the ensemble is recast as a low-rank matrix recovery problem from linear measurements. The architectures we are considering impose a certain type of structure on the linear operators. Although our results depend on the mixing forms being random, this imposed structure results in a very different type of random projection than those analyzed in the low-rank recovery literature to date.

==> notations.tex <==
%\newcommand{\vm}[1]{\boldsymbol{#1}}
\renewcommand{\P}[1]{\operatorname{P}\left\{#1\right\}}
\newcommand{\E}{\operatorname{E}}
%\newcommand{\tr}[1]{\operatorname{trace}\left(#1\right)}
\newcommand{\Tr}[1]{\operatorname{trace}\left(#1\right)}
\newcommand{\rank}[1]{\operatorname{rank}\left(#1\right)}
%\DeclareMathOperator{\vc}{vec}
%\DeclareMathOperator{\Prob}{P}
%\newcommand{\argmin}{\operatorname{argmin}}
\renewcommand{\H}{{\operatorname{H}}}
\newcommand{\T}{{\operatorname{T}}}


\newcommand{\er}{\mathrm{e}}
\renewcommand{\j}{\mathrm{j}}
\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

%\def\D{\Delta}
%\def\si{\vm{\Psi}}
%\def\y{\vm{Y}}
%\def\x{\vm{X}}
%\def\u{\boldsymbol{U}}
%\def\v{\boldsymbol{V}}
%\def\e{\vm{e}}
%\def\eb{\bar{\vm{e}}}
%\def\a{\vm{A}}
%\def\A{\vm{A}}
%\def\i{\vm{I}}
%\def\f{\vm{F}}
%\def\p{\vm{P}}
%\def\q{\vm{Q}}
%\def\h{\vm{H}}
%\def\A{\vm{A}}
%\def\z{\vm{Z}}
%\def\w{\vm{W}}
%\def\G{\vm{G}}
%\def\ss{\vm{Sigma}}
%\def\fy{\vm{\Phi}}
%\def\k{\kappa}
%\def\ss{\vm{\Sigma}}
%\def\aa{\vm{a}}
%\def\ff{\vm{f}}
%\def\O{\Omega}
%\def\o{\omega}
%\def\d{\vm{d}}
%\def\op{\nu}
\def\zz{\vm{z}}
%
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\xx}{\vct{x}}
\newcommand{\ww}{\vct{w}}
\newcommand{\Bmat}{\mtx{B}}
\newcommand{\Cmat}{\mtx{C}}
\newcommand{\mm}{\vct{m}}
\newcommand{\hh}{\vct{h}}
\newcommand{\yy}{\vct{y}}
\newcommand{\yh}{\hat{\yy}}
\newcommand{\tF}{\tilde{\mtx{F}}}
\newcommand{\tFs}{\tilde{F}}
\newcommand{\Ak}{\mtx{A}_k}
\newcommand{\bk}{\hat{\vct{b}}_k}
\newcommand{\ck}{\hat{\vct{c}}_k}
\newcommand{\I}{\mtx{I}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Zk}{\mtx{Z}_k}
\newcommand{\vk}{\vct{v}_k}
\newcommand{\uk}{\vct{u}_k}
\newcommand{\uu}{\vct{u}}
\newcommand{\vv}{\vct{v}}
\newcommand{\cZ}{\mathcal{Z}}

%
%
%
%
\def\PT{\mathcal{P}_T}
\def\PTc{\mathcal{P}_{T^\perp}}
\def\cA{\mathcal{A}}
%\def\cB{\mathcal{B}}
%\def\cL{\mathcal{L}}
%\def\reals{\mathbb{R}}
%\def\comps{\mathbb{C}}
%\def\g{\gamma}
%\def\ap{\alpha}
%\def\be{\beta}
%\def\t{\vm{\Theta}}
%\def\b{\vm{B}}


\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
